ParsiNLU: A Suite of Language Understanding Challenges for Persian

Despite the progress made in recent years in addressing natural language understanding (NLU) challenges, the majority of this progress remains to be concentrated on resource-rich languages like English. This work focuses on Persian language, one of the widely spoken languages in the world, and yet there are few NLU datasets available for this rich language. The availability of high-quality evaluation datasets is a necessity for reliable assessment of the progress on different NLU tasks and domains. We introduce ParsiNLU, the first benchmark in Persian language that includes a range of high-level tasks -- Reading Comprehension, Textual Entailment, etc. These datasets are collected in a multitude of ways, often involving manual annotations by native speakers. This results in over 14.5$k$ new instances across 6 distinct NLU tasks. Besides, we present the first results on state-of-the-art monolingual and multi-lingual pre-trained language-models on this benchmark and compare them with human performance, which provides valuable insights into our ability to tackle natural language understanding challenges in Persian. We hope ParsiNLU fosters further research and advances in Persian language understanding.

==> old_abstract.tex <==
  \begin{comment}
%% try 2: 
The progress of past few years in language technologies has enabled the field to address more challenging natural language understanding (NLU) tasks. 
  Such technological breakthroughs would have been merely impossible without the existence of high-quality and challenging tasks for language understanding.  
%% abstract v1 
%   Persian is one of the widely spoken languages in the world, yet there are virtually no quality resources of high-level NLP tasks for this rich language.
Persian is one of the widely spoken languages in the world, yet there is little resources available for this rich language. 
  \ac{are we sure about this statement?} \daniel{better? Alternatively, how else can we open the abstract?}
  In this work we introduce \parsiglue, a comprehensive suit of high-level NLP tasks, for Persian language \ac{maybe we should say ``the first comprehensive''}. 
  This suit contains 6 different key NLP tasks --- \emph{Reading Comprehension} (RC), \emph{Multiple-Choice Question-Answering} (MC), \emph{Textual Entailment} (TE), \emph{Sentiment Analysis} (SA), \emph{Query Paraphrasing} (QP) and \emph{Machine Translation} (MT). 
  The data collection of the tasks involve various techniques, such as expert translation, direct annotation of the tasks or using existing sources of supervision. 
  Overall, \parsiglue\ contains more than xx$k$ instances across all the tasks, $xx$\% of which are collected in this work. 
  We benchmark a range of state-of-the-art models on this novel dataset, revealing that current methods based on multilingual pretraining ... . 
  This is unique language resource for Persian in several respects, which hopefully will foster more future research on this rich language and its unique attributes. \ac{maybe we can motivate this from a different angle. saying that ParsiGLUE is the first comprehensive persian NLU dataset and previous works were focused on single task on a narrow domain. e.g.,
  ``To measure the progress on an effective NLU model for Persian, it is critical to have an evaluation corpus that can assess the quality of the model on a range of different linguistic tasks in different domains. ParsiGLUE is the first corpus in Persian language that attempts achieving this goal. It includes a wide range of key NLP tasks --- \emph{Reading Comprehension} (RC) [...] ''}\footnote{
    https://github.com/persiannlp/parsiglue
    \label{github-link}  }
  \end{comment}s
